Reflectivity Is All You Need!: Advancing LiDAR Semantic Segmentation

LiDAR semantic segmentation frameworks predominantly use geometry-based features to differentiate objects within a scan. Although these methods excel in scenarios with clear boundaries and distinct shapes, their performance declines in environments where boundaries are indistinct, particularly in off-road contexts. To address this issue, recent advances in 3D segmentation algorithms have aimed to leverage raw LiDAR intensity readings to improve prediction precision. However, despite these advances, existing learning-based models face challenges in linking the complex interactions between raw intensity and variables such as distance, incidence angle, material reflectivity, and atmospheric conditions. Building upon our previous work, this paper explores the advantages of employing calibrated intensity (also referred to as reflectivity) within learning-based LiDAR semantic segmentation frameworks. We start by demonstrating that adding reflectivity as input enhances the LiDAR semantic segmentation model by providing a better data representation. Extensive experimentation with the Rellis-3d off-road dataset shows that replacing intensity with reflectivity results in a 4\% improvement in mean Intersection over Union (mIoU) for off-road scenarios. We demonstrate the potential benefits of using calibrated intensity for semantic segmentation in urban environments (SemanticKITTI) and for cross-sensor domain adaptation. Additionally, we tested the Segment Anything Model (SAM) using reflectivity as input, resulting in improved segmentation masks for LiDAR images.

==> figures/angle_inci.tex <==
\begin{figure}
    \centering
    \includegraphics[width = 0.45\textwidth]{images/lidar_int.eps}
    \caption{Interaction of laser beam with the surface at a different angle of incidence.}
    \label{fig:angle_inci}
\vspace{-0.5 cm}
\end{figure}

==> figures/irn_proj.tex <==
\begin{figure*}[h]
    \centering
    \vspace{0.2 cm}
    \includegraphics[width = 0.95\textwidth]{images/irn.eps}
    \caption{Spherical projection of a) Raw intensity data b) Calibrated intensity for Range and angle of incidence($\alpha$) c) Calibrated intensity for near-range ($\eta$), range and angle of incidence($\alpha$).}
    \label{fig:irn_proj}
\vspace{-0.5 cm}
\end{figure*}

==> sections/inference_old.tex <==
\section{Inference}
The experiments carried out on the Rellis-3D and SemanticKITTI datasets indicate that utilizing reflectivity rather than intensity yields improved segmentation results in both off-road and on-road contexts. The notable enhancement in accuracy observed in off-road scenes can be attributed to the reflectivity parameter's ability to distinguish between classes. This is particularly crucial as objects within the same class maintain consistent color and texture, while variations exist across different classes. Given the unstructured nature of off-road environments and the presence of loose boundaries, relying solely on geometry-based features resulted in lower performance.  

In urban settings, where boundaries are clearly delineated across scenes, geometric features play a more significant role in learning compared to reflectivity/intensity parameters. Additionally, variations in intensity values between objects, such as different intensity values for cars based on surface color and texture, can also impact segmentation results. These factors may contribute to the limited improvement observed when using reflectivity in SemanticKITTI experiments. However, it should be noted that the incorporation of reflectivity consistently led to enhanced segmentation results compared to intensity across all experiments.

After conducting cross-sensor experiments on the Rellis-3D dataset, it is clear that transferring a model from one sensor to another, even within the same scene, produces unsatisfactory outcomes. Although LiDAR intensity calibration has been effective in enhancing results, other factors such as the number of rings, ray pattern, and field of view have notable impacts on cross-domain capability.


==> sections/introduction_old.tex <==
\section{introduction}
LiDAR (light detection and ranging) segmentation has become a crucial technology in autonomous driving and robotics, providing a detailed three-dimensional perspective of the surrounding environment. This process involves categorizing each point in a LiDAR point cloud into distinct classes, such as vehicles, pedestrians, trees, and buildings, allowing machines to perceive and interact with their environments. In autonomous vehicles, LiDAR semantic segmentation is essential for obstacle detection, navigation, and path planning, facilitating informed decisions in complex and dynamic contexts.% The integration of this technology ensures autonomous systems can operate safely and efficiently in human-centric environments, driving the evolution of intelligent systems in our increasingly automated society.

However, traditional learning-based LiDAR semantic segmentation models have focused primarily on the geometric characteristics of objects. For example, deep learning models like SalsaNext \cite{10.1007/978-3-030-64559-5_16} \cite{9304694} utilize encoder-decoder architectures to analyze raster laser scan images, where four of five channels convey geometry information ($range, x, y, z$). Meanwhile, Cylinder3D \cite{zhu2020cylindrical}  employs 3D sparse convolution operations to probe the 3D topology of the laser scan through cylindrical partitioning, leveraging 3D geometric characteristics to extract semantic features. Although these approaches are effective in urban settings with distinct edges and shapes, they can face challenges in more complex, unstructured off-road environments. Notably, both models incorporate the LiDAR return's intensity as an auxiliary input to enhance learning. However, these intensity values, which are influenced by factors such as range, incidence angle, and surface characteristics, are not well calibrated, leading to a distortion of meaningful information. Calibrating intensity values in LiDAR data by eliminating dependencies on range and angle of incidence and focusing solely on reflectivity represents an object correlating their ability to reflect radiation. When this calibration is done accurately, it can significantly enhance the visual quality of projected LiDAR data, providing finer-grained and more insightful details (see Fig. \ref{fig:irn_proj}).
%\input{figures/msalsanext} 
It should be noted that in this paper, \textit{calibrated intensity} and \textit{reflectivity} are used interchangeably to refer to a parameter distinct from the raw intensity.

Research on LiDAR intensity has been carried out predominantly in the geospatial area, focusing on segmenting aerial LiDAR scans to discern different features such as vegetation, buildings and roads \cite{rs12101677} \cite{s22176388}. In terrestrial laser scanning, calibrated intensity data prove crucial for applications such as urban roadway lane detection and vegetation monitoring \cite{electronics7110276} \cite{9246255}. The calibration of intensity for improved reflectivity measurement has thus become a key research objective aimed at enhancing the interpretation of sensor data. In particular, research has introduced innovative approaches for data collection and calibration; \cite{6849466}  proposed a novel design for collecting sample data in controlled environments to estimate parameters for a customized range-intensity equation for terrestrial laser scanners. \cite{4432711} Outlined a new empirical calibration method for the intensity of laser scanners, using brightness targets and a calibrated reference panel under both laboratory and field conditions.
\begin{figure}[!t]
    \centering
    \vspace{0.2 cm}
    \includegraphics[width = 0.45\textwidth, height = 5.5 cm]{images/gradd_irn.eps}
    \caption{Comparison of raw intensity versus range for the grass class. The figure demonstrates how intensity varies with the range and angle of incidence. It highlights the relationship between angle of incidence and intensity, indicating that the greatest intensity at each range is achieved when $\alpha$ nears 0, while the lowest intensity occurs when $\alpha$ is approximately $\pi/2$.}
    \label{fig:raw_data}
\vspace{-0.5 cm}
\end{figure}
However, these studies have largely concentrated on terrestrial laser scanners, with mobile LiDAR systems, extensively used in autonomous vehicles and robotics, receiving less attention. 

Datasets widely recognized in the field, such as SemanticKITTI\cite{behley2019iccv} or Rellis-3D\cite{9561251}, often feature raw LiDAR data. To address this gap, recent efforts have been made to explore the calibrated intensity of mobile LiDAR. Our previous work \cite{10.1007/978-3-031-63596-0_54} introduced a hybrid method for calibrating intensity values based on range and incidence angle, demonstrating its utility for object segmentation in off-road environments. However, the exploration primarily assessed the advantages of calibrated intensity with conventional clustering algorithms and a limited array of object classes. A significant limitation of traditional methods is their struggle with high-dimensional data, which can result in inaccuracies when clustering complex multi-object scenes.

Advancing from the foundation, this paper explores the combination of reflectivity data with geometric details to augment existing deep-learning models for broader class categorization. This research introduces a novel approach that fuses reflectivity data with neural network models to further refine segmentation. Using the detailed insights offered by reflectivity values, we aim to establish a more enhanced data representation for LiDAR semantic segmentation capable of addressing the intricacies of off-road terrains. Furthermore, with the emergence of foundation models such as Segment Anything \cite{kirillov2023segment}, our aim is to utilize enhanced reflectivity data to generate segmentation masks using prompts. This approach advances us towards automating the labor-intensive task of LiDAR annotation. Our findings reveal that incorporating reflectivity data considerably improves the performance of existing LiDAR semantic segmentation models, indicating a promising pathway for future advancements in the field. The primary contributions of this work are:
\begin{itemize}
    \item Data-driven approach for calibrating near-range intensity measurements.
    \item LiDAR reflectivity as an input feature for enhanced data representation with respect to the current state-of-the-art segmentation models.
    \item Using reflectivity learning through the SalsaNext model shows a boost in segmentation performance.
    \item Generation of segmentation masks from Segment Anything using Range, Intensity, and Reflectivity as input.
    \item A unified LiDAR intensity representation to enable cross-sensor calibration, thereby improving domain adaptation capabilities.
\end{itemize}




==> sections/related_work.tex <==
\section{related work}
\textbf{Semantic Segmentation: }LiDAR semantic segmentation has been a widely researched area in the perception domain. The majority of the work relies on extracting geometry and intensity-based features from point clouds through convolutions in order to segment objects in the scene. Deep learning based algorithms such as SalsaNext \cite{10.1007/978-3-030-64559-5_16} employ encoder-decoder architecture on the raster image (range, $x, y, z$, intensity) of the laser scan whereas Cylinder3D \cite{zhu2020cylindrical} utilize the 3D topology of the laser scan through the cylinder partition extracting the semantic features.

\textbf{LiDAR intensity calibration:} Most segmentation frameworks use the LiDAR return, i.e., intensity, to extract features. The intensity of LiDAR scans depends on various factors, majorly range, angle of incidence, and reflectivity, as shown in Figure \ref{fig:angle_inci}. The reflectivity parameter corresponds directly to the object's ability to reflect radiation. Previous works \cite{6849466}\cite{4432711} calibrate intensity using a model-driven approach with controlled experimental setups. Our previous work \cite{10.1007/978-3-031-63596-0_54} calibrates the intensity values for the range and angle of incidence using a hybrid approach that combines model and data-driven methodologies, thus demonstrating the ability to segment out a limited number of objects using traditional clustering methods. 
\begin{figure}
    \centering
    \includegraphics[width = 0.5\textwidth]{images/Angleofincidence.png}
    \caption{Interaction of laser beam with the surface at a different angle of incidence. (Image adapted from previous work \cite{10.1007/978-3-031-63596-0_54}).}
    \label{fig:angle_inci}
\end{figure}
Through this paper, we try to focus on employing reflectivity as a direct input to Deep Learning architectures in order to capture rich details and evaluate them using raw intensity. 


%\textbf{Cross Domain Adaptation:} The paradigm of cross-domain adaptation has been of important research in robotic perception. The ability of a model to transfer knowledge learned from one dataset(source) to another(target) dataset proves the architecture's resilience. However different datasets may have variations in sensor characteristics and scene compositions. The sensor characteristics primarily include ray pattern and intensity format. Certain sensors employ a fitting function on the raw intensity values in order to calibrate, thereby minimizing intensity-feature-based knowledge transfer. This work also concentrates on converting different intensity formats to a generalized LiDAR equation-based format, thereby enabling improved domain adaptation.

==> table/combine.tex <==
\begin{table*}[!ht]
    \centering
    \vspace{0.2 cm}
    \fontsize{7pt}{9pt}\selectfont
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
         \hline
         Dataset & Config & Grass & Tree & Pole & Vehicle & Log & Person & Fence & Bush & Concrete & Barrier & Puddle & Mud & Rubble & MIoU \\
         \hline
         \multirow{4}{*}{\rotatebox[origin=c]{90}{Rellis-3D}}& rxyzi & 35.1 & 49.6 & \textbf{56.1} & \textbf{23.8} & \textbf{14.5} & 62.8 & 0.6 & 30.2 & 50.0 & 80.1 & 20.4 & 10.7 & 66.6 & 38.4\\ \cline{2-16}
           & rxyzn & \textbf{37.6} & 55.7 & 52.3 & 21.4 & 10.3 & 76.0 & 1.4 & 33.9 & \textbf{74.5} & \textbf{81.3} & \textbf{25.0} & \textbf{13.7} & 67.7 & \textbf{42.4}\\ \cline{2-16}
         %\hline
          & rxyzirn & 36.2 & 55.8  & 51.0 & 20.3 & 9.9 & \textbf{82.7} & 2.7 &  34.0 & 60.1 & 79.1 & 22.6 & 12.9 & \textbf{68.9} & 41.2\\ \cline{2-16}
         %\hline
          & rxyzi$\_$gau & 36.0 & \textbf{58.4} & 52.5 & 22.2 & 12.6 & 82.6 & \textbf{3.2} & \textbf{35.7} & 59.9 & 80.9 & 24.2 & 12.5 & 63.8 & 41.9\\
         \hline
         \hline
         Source & Target & Grass & Tree & Pole & Vehicle & Log & Person & Fence & Bush & Concrete & Barrier & Puddle & Mud & Rubble & MIoU \\
         \hline
         OS rxyzi & VLP rxyzi & 19.6 & \textbf{40.3} & 0.1 & 0.0 & 0.0 & 2.1 & 0.0 & 33.9 & 1.7 & 0.0 & 0.0 & 0.3 & 0.2 & 7.5 \\ 
         \hline
          OS rxyzn & VLP rxyzn & \textbf{30.3} & 38.3 & \textbf{1.1} & \textbf{4.8} & \textbf{0.2} & \textbf{34.1} & \textbf{0.9} & \textbf{35.4} & \textbf{27.3} & \textbf{3.8} & \textbf{1.6} & \textbf{0.9} & \textbf{0.3} & \textbf{13.8}\\ 
         \hline
    \end{tabular}
    %\vspace{0.4 cm}
    \caption{mIoU of experiment results on Rellis-3D with different input configuration and cross-sensor adaptation}
    \label{tab:combine_results}
    \vspace{-0.4 cm}
\end{table*}
